BVRI Photometric Calibration of the Nedeljkovi\'c Telescope

We have done photometric calibration of the 60 cm Nedeljkovi\'{c} telescope equipped with FLI PL 230 CCD camera, mounted at the Astronomical Station Vidojevica (Serbia), using standard stars from the Landolt's catalog. We have imaged 31 fields of standard stars using Johnson's $BVRI$ filters during three nights in August 2019. We have measured both extinction and color correction. Relating our calibrated magnitudes to the magnitudes of the standard stars from the Landolt's catalog, we have achieved accuracy of 2\%-5\% for the $BVRI$ magnitudes.

==> abr_saj.tex <==
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&ARv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting 
%Abstracts
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\ao{ApOpt}%   % Applied Optics ++
\newcommand\apj{ApJ}%    % Astrophysical Journal ++
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics 
%Research 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\bac{Bull. astr. Inst. Czechosl.}
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical 
%Society/Division for Planetary Sciences Meeting Abstracts
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\icarus{Icar}% % Icarus
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{JGR}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and 
%Radiative Trasfer 
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\nat{Natur}%  % Nature 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics ++
\newcommand\prb{PhRvB}% % Physical Review B: Solid State ++
\newcommand\prc{PhRvC}% % Physical Review C ++
\newcommand\prd{PhRvD}% % Physical Review D ++
\newcommand\pre{PhRvE}% % Physical Review E ++
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 





==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.6em{\hfil.\hfil}%
\setbox8=\hbox to0.5em{\hfil$^{#1}$\hfil}%
\box7\kern-0.5em\box8}}

\def\dan{\point{\rm d}}
\def\cas{\point{\rm h}}
\def\minut{\point{\rm m}}
\def\sekund{\point{\mathrm{s}}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



